Factorization Machines with Regularization for Sparse Feature Interactions

Factorization machines (FMs) are machine learning predictive models based on second-order feature interactions and FMs with sparse regularization are called sparse FMs. Such regularizations enable feature selection, which selects the most relevant features for accurate prediction, and therefore they can contribute to the improvement of the model accuracy and interpretability. However, because FMs use second-order feature interactions, the selection of features often causes the loss of many relevant feature interactions in the resultant models. In such cases, FMs with regularization specially designed for feature interaction selection trying to achieve interaction-level sparsity may be preferred instead of those just for feature selection trying to achieve feature-level sparsity. In this paper, we present a new regularization scheme for feature interaction selection in FMs. The proposed regularizer is an upper bound of the $\ell_1$ regularizer for the feature interaction matrix, which is computed from the parameter matrix of FMs. For feature interaction selection, our proposed regularizer makes the feature interaction matrix sparse without a restriction on sparsity patterns imposed by the existing methods. We also describe efficient proximal algorithms for the proposed FMs and present theoretical analyses of both existing and the new regularize. In addition, we will discuss how our ideas can be applied or extended to more accurate feature selection and other related models such as higher-order FMs and the all-subsets model. The analysis and experimental results on synthetic and real-world datasets show the effectiveness of the proposed methods.

==> Factorization machines with Regularization for Sparse Feature Interactions/additional_experiments.tex <==
\section{Additional Experiments}
\subsection{Efficiency Comparison on Real-world Dataset}
    \label{subsec:efficiency_real_world}
    \begin{figure*}[t]
        \centering
        \subfloat[ML100K Dataset with $\tilde{\lambda}_p=10^{-4}$ (left) and $10^{-5}$ (right).]{
        \includegraphics[width=80mm]{ml100k/exact_objective_gamma0.0001.pdf}
        \includegraphics[width=80mm]{ml100k/exact_objective_gamma1e-05.pdf}
        \label{fig:exact_ml100k}
        }\\
        \subfloat[a9a Dataset with $\tilde{\lambda}_p=10^{-4}$ (left) and $10^{-5}$ (right).]{
        \includegraphics[width=80mm]{a9a/exact_objective_gamma0.0001.pdf}
        \includegraphics[width=80mm]{a9a/exact_objective_gamma1e-05.pdf}
        \label{fig:exact_a9a}
        }
        \caption{Trajectories of $\norm{\bm{W}}_1$ regularized objective value for \textbf{TI}, \textbf{CS}, \textbf{L21}, \textbf{L1}, \textbf{$\Omega_*$-nmAPGD}, \textbf{$\Omega_*$-SubGD}, and \textbf{SLQR} methods on (a) ML100K dataset and (b) a9a dataset.}
        \label{fig:exact_real}
    \end{figure*}

    We evaluated the efficiency of the proposed and existing methods on the ML100K dataset and the a9a dataset as in~\cref{subsubsec:efficiency}.
    We ran the experiment with $\tilde{\lambda}_p=10^{-4}$ and $10^{-5}$ on both datasets.
    We set $\lambda_p = \lambda_{\mathrm{tr}}=10^{-4}$ on the ML100K dataset and $\lambda_p=\lambda_{\mathrm{tr}}=10^{-3}$ on the a9a dataset.
    The other settings are the same those in~\cref{subsubsec:efficiency}.
    Because we compared the convergence speeds of objective values, we didn't separate datasets to training, validation, and testing datasets, i.e., we used $100,000$ and $48,642$ instances for training on the ML100K and the a9a datasets, respectively.
    
    As shown in~\cref{fig:exact_ml100k}, \textbf{TI} and \textbf{CS} converged much faster than the other methods in terms of $\Omega_*$ ($\norm{\bm{W}}_1$) regularized objective function on both the ML100K dataset and the a9a dataset.
    These results indicate that the proposed regularizers can be good alternative to $\Omega_*$ for not only synthetic datasets but also some real-world datasets.
    
\subsection{Optimization Methods Comparison}
    \label{subsec:solver}
    We compared the convergence speeds of the some algorithms for TI-sparse FMs and CS-sparse FMs on both synthetic and real-world datasets.
    We ran this experiment on an Arch Linux desktop with an Intel Core i7-4790 (3.60 GHz) CPU and 16 GB RAM.
    
    \paragraph{Methods Compared.}
    We compared the following algorithms for TI-sparse FMs and CS-sparse FMs:
    \begin{itemize}
        \item \textbf{PCD}: the proximal coordinate descent algorithm (only TI-sparse FMs).
        \item \textbf{PBCD}: the proximal block coordinate descent algorithm (only CS-sparse FMs).
        \item \textbf{APGD}: FISTA with restart.
        \item \textbf{nmAPGD}: the non-monotone APGD algorithm~\citep{li2015accelerated}.
        \item \textbf{PSGD}: the PSGD algorithm.
        \item \textbf{MB-PSGD}: the mini-batch PSGD algorithm (only on real-world datasets).
        \item \textbf{Katyusha}: the Katyusha algorithm proposed by~\citet{allen2017katyusha}. It is similar to an accelerated proximal stochastic variance reduction gradient algorithm~\citep{nitanda2014stochastic} but introduces an additional moment term, which is called Katyusha momentum.
        \item \textbf{MB-Katyusha}: the mini-batch Katyusha algorithm (only on real-world datasets).
    \end{itemize}
    We used line search techniques for the step size in \textbf{APGD} and \textbf{nmAPGD}~\citep{beck2009fast,li2015accelerated} but we did not use them in \textbf{PCD} and \textbf{PBCD} because their sub-problems are smooth.
    For the (mini-batch) PSGD-based algprithms, we ran the experiment using initial step size $\eta_{0}=1.0$, $0.1$ and $0.01$ but we show only the best results.
    In \textbf{PSGD} and \textbf{MB-PSGD}, rather than using a constant step size, we used a diminishing step size as proposed by~\citet{bottou2012stochastic}: $\eta = \eta_{0}(1+\eta_0 \lambda_p t)^{-1}$ at the $t$-th iteration.
    On the other hand, \textbf{Katyusha} and \textbf{MB-Katyusha} used a constant step size: $\eta=\eta_0$.
    In \textbf{MB-PSGD} and \textbf{MB-Katyusha}, we set the number of instances in one mini-batch $N_b$ to be $Nd / \nnz{\bm{X}}$, which reduces the computational cost per epoch from $O(NdK)$ to $O(\nnz{\bm{X}}k)$.
    For the evaluation of the proximal operator~\eqref{eq:prox_ti}, we used~\cref{alg:prox_ti_randomize}, which runs in $O(d)$ time in expectation.
    \begin{figure}[t!]
        \centering
        \subfloat[Feature interaction selection setting: $d_{\mathrm{true}}=80$, $b=8$ and $d_{\mathrm{noise}}=20$ with $N=200$ and $20,000$ for \textbf{TI} method.]{
        \includegraphics[width=80mm]{synthetic/runtime_n200_gamma0.1.pdf} 
        \includegraphics[width=80mm]{synthetic/runtime_n20000_gamma0.1.pdf}
        \label{fig:synthetic_solver_feature_interaction_selection}
        }\\
        \subfloat[Feature selection setting: $d_{\mathrm{true}}=20$, $b=1$ and $d_{\mathrm{noise}}=80$ with $N=200$ (left) and $20,000$ for \textbf{TI} method.]{
        \includegraphics[width=80mm]{synthetic_feature_wise/ti_runtime_n200_gamma0.1.pdf} 
        \includegraphics[width=80mm]{synthetic_feature_wise/ti_runtime_n20000_gamma0.1.pdf}
        \label{fig:synthetic_solver_feature_selection}
        }\\
        \subfloat[Feature selection setting: $d_{\mathrm{true}}=20$, $b=1$ and $d_{\mathrm{noise}}=80$ with $N=200$ (left) and $20,000$ for \textbf{CS} method.]{
        \includegraphics[width=80mm]{synthetic_feature_wise/cs_runtime_n200_gamma0.1.pdf} 
        \includegraphics[width=80mm]{synthetic_feature_wise/cs_runtime_n20000_gamma0.1.pdf}
        \label{fig:synthetic_solver_feature_selection_cs}
        }
        \caption{Runtime comparisons among \textbf{PCD}, \textbf{PBCD}, \textbf{APGD}, \textbf{nmAPGD}, \textbf{PSGD}, and \textbf{Katyusha} algorithms on synthetic datasets using different amounts of training data: (a) feature interaction selection setting datasets for \textbf{TI} method; (b) feature selection setting datasets for \textbf{TI} method; (c) feature selection setting datasets for \textbf{CS} method. Left and right graphs show results for datasets with $N=200$ and $20,000$, respectively.}
        \label{fig:synthetic_solver}
    \end{figure}
    
    \begin{figure}[t!]
        \centering
        \subfloat[ML100K dataset ($N=100,000$): \textbf{TI} method (left) and \textbf{CS} method (right) with $\lambda_w = 5\times 10^{-4}$, $\lambda_p = 5\times 10^{-5}$, and $\tilde{\lambda}_p = 5\times 10^{-5}$.]{
        \includegraphics[width=80mm]{ml100k/runtime_ti.pdf} 
        \includegraphics[width=80mm]{ml100k/runtime_cs.pdf}
        \label{fig:solver_ml100k}
        }\\
        \subfloat[a9a dataset ($N=48,842$): \textbf{TI} method (left) and \textbf{CS} method (right) with $\lambda_w = 5\times 10^{-2}$, $\lambda_p = 5\times 10^{-4}$, and $\tilde{\lambda}_p = 5\times 10^{-4}$.]{
        \includegraphics[width=80mm]{a9a/runtime_ti.pdf} 
        \includegraphics[width=80mm]{a9a/runtime_cs.pdf}
        \label{fig:solver_a9a}
        }\\
        \caption{Runtime comparisons among \textbf{PCD}, \textbf{PBCD}, \textbf{APGD}, \textbf{nmAPGD}, \textbf{PSGD}, \textbf{MB-PSGD}, \textbf{Katyusha}, and \textbf{MB-Katyusha} algorithms on (a) ML100K dataset and (b) a9a dataset. Left and right graphs show results for \textbf{TI} and \textbf{CS} method, respectively.}
        \label{fig:solver_real}
    \end{figure}
    
    \paragraph{Datasets.}
    We used feature interaction selection setting datasets, feature selection setting datasets, the ML100K dataset, and the a9a dataset.
    We set the number of instances of synthetic datasets $200$ and $20,000$ in order to compare scalabilities of algorithms w.r.t $N$.
    As in~\cref{subsec:efficiency_real_world}, we used $100,000$ and $48,642$ instances for training on the ML100K and the a9a datasets, respectively.
    We ran the experiment ten times using different initial random seeds.
    On synthetic datasets, we set $\lambda_{p}=\tilde{\lambda_p}=0.1$ for the batch algorithms (\textbf{PCD}, \textbf{PBCD}, \textbf{APGD}, and \textbf{nmAPGD}).
    For the stochastic algorithms (\textbf{PSGD} and \textbf{Katyusha}), we first scaled the feature vectors and targets: we used $\bm{x}_n / \sqrt{d}$ and $y_n / d$ as feature vectors and targets and set $\lambda_p$ and $\tilde{\lambda}_p$ to $0.1/d^2$.
    Since we used the squared loss and $f_{\mathrm{FM}}(\bm{x}/\sqrt{d}; \bm{0}, \bm{P}) = f_{\mathrm{FM}}(\bm{x}; \bm{0}, \bm{P})/d$, the balance between the loss term and regularization term was the same as that in the batch algorithms.
    On the ML100K dataset, we set $\lambda_w=0.5 \times 10^{-4}$, $\lambda_p=0.5 \times 10^{-4}$, and $\tilde{\lambda}_p = 0.5 \times 10^{-4}$ for all methods.
    On the a9a dataset, we set $\lambda_w=0.5 \times 10^{-2}$, $\lambda_p=0.5 \times 10^{-3}$, and $\tilde{\lambda}_p = 0.5 \times 10^{-3}$ for all methods.
    They were chosen based on the results in~\cref{subsec:real}.
    
    \paragraph{Results: batch vs stochastic.}
    As shown in~\cref{fig:synthetic_solver}, on synthetic datasets, when the number of training instances was $20,000$, the stochastic algorithms (\textbf{PSGD} and \textbf{Katyusha}) were faster than the batch algorithms (\textbf{PCD}, \textbf{PBCD}, \textbf{APGD}, and \textbf{nmAPGD}).
    This indicates that stochastic algorithms can be more useful than batch algorithms for large-scale dense datasets, as described in~\cref{subsec:pgd_ti} and~\cref{subsec:pgd_cs}.
    However, the stochastic algorithms take $O(dk)$ time at each iteration even if a sampled feature vector is sparse.
    On synthetic datasets, the feature vectors were dense since they were generated from Gaussian distributions, so the stochastic algorithms might be relatively slower in some real-world applications.
    Indeed, as shown in~\cref{fig:solver_real}, on real-world datasets, the completely stochastic algorithms (\textbf{PSGD} and \textbf{Katyusha}) were not faster than batch algorithms although although $N \gg d$ on both datasets.
    The use of appropriate size mini-batch improved the convergence speed as our expected: \textbf{MB-PSGD} and \textbf{MB-Katyusha} were faster than their completely stochastic versions.
    Nevertheless, such mini-batch algorithms were slower than \textbf{PCD} and \textbf{PBCD} on the ML100K dataset and the \textbf{PCD} on the a9a dataset.
    Moreover, performances of (mini-batch) stochastic algorithms were sensitive w.r.t the choice of the step size hyperparameter and the objective values usually diverged with $\eta_0=1.0$.
    Thus, as our analysis in~\cref{subsec:pgd_ti}, the PSGD-based algorithms should be used only when $\nnz{\bm{X}}/d$ is large.
    Note that $\nnz{\bm{X}}/d$ of the ML100K and the a9a datasets in this experiment are $338$ and $5,506$, respectively (clearly, on synthetic datasets $\nnz{\bm{X}}/d = N$).

    \paragraph{Results: \textbf{PCD}/\textbf{PBCD} vs \textbf{APGD}/\textbf{nmAPGD}.}
    On synthetic datasets (\cref{fig:synthetic_solver}), \textbf{PCD}/\textbf{PBCD}, \textbf{APGD}, and \textbf{nmAPGD} tended to show similar results but \textbf{PCD} was much faster than \textbf{APGD} and \textbf{nmAPGD} on the feature interaction selecting dataset with $N=200$.
    On real-world datasets (\cref{fig:solver_real}), \textbf{PCD} and \textbf{PBCD} were much faster than \textbf{APGD} and \textbf{nmAPGD}.
    Strictly speaking, not PCD-based algorithms but PGD/PSGD-based algorithms should be used since \textbf{TI} (\textbf{CS}) regularizer is not seperable w.r.t each coordinate (each row vector) in $\bm{P}$.
    However, our results indicate that \textbf{PCD} and \textbf{PBCD} can work better than \textbf{nmAPGD} and \textbf{APGD} practically.
    Moreover, again, \textbf{PCD} and \textbf{PBCD} have some important practical advantages: (i) easy to implement, (ii) easy to extend to related models (as shown in~\cref{sec:extension}), and (iii) having few hyperparameters.
    
\subsection{Comparison of~\cref{alg:prox_ti_sort} and~\cref{alg:prox_ti_randomize}}
    We compared two algorithms for the proximal operator~\eqref{eq:prox_ti},~\cref{alg:prox_ti_sort} (\textbf{Sort}) and~\cref{alg:prox_ti_randomize} (\textbf{Random}) proposed by~\citet{filipe2011online}.
    For a $d$-dimensional vector, \textbf{Sort} and \textbf{Random} run in $O(d \log d)$ time and $O(d)$ time, respectively.
    We evaluated the runtime of two algorithms for a $d$-dimensional vector generated from a Gaussian distribution, $\mathcal{N}(\bm{0}, \sigma^2 \eye_{d})$ with varying $d \in \{2^{3}, 2^{4}, \ldots, 2^{14}\}$.
    We set $\sigma=1.0$ and $\sigma=10.0$ and the regularization strength $\lambda=0.001$, $\lambda=0.1$, and $\lambda=10.0$.
    We ran the experiment $100$ times with different initial random seeds and report the average runtimes.
    For \textbf{Sort}, we used Nim's standard \texttt{sort} procedure, which is an implementation of merge sort.
    
    \begin{figure}[t]
        \centering
        \subfloat[$\sigma=1.0$.]{
        \includegraphics[width=52mm]{proximal/proximal_algorithm_comparison_std1.0_lam0.001.pdf}
        \includegraphics[width=52mm]{proximal/proximal_algorithm_comparison_std1.0_lam0.1.pdf}
        \includegraphics[width=52mm]{proximal/proximal_algorithm_comparison_std1.0_lam10.0.pdf}
        \label{fig:prox_sort_vs_random_std1.0}
        }\\
        \subfloat[$\sigma=10.0$.]{
        \includegraphics[width=52mm]{proximal/proximal_algorithm_comparison_std10.0_lam0.001.pdf}
        \includegraphics[width=52mm]{proximal/proximal_algorithm_comparison_std10.0_lam0.1.pdf}
        \includegraphics[width=52mm]{proximal/proximal_algorithm_comparison_std10.0_lam10.0.pdf}
        \label{fig:prox_sort_vs_random_std10.0}
        }
        \caption{Comparison of~\cref{alg:prox_ti_sort} (\textbf{Sort}) and~\cref{alg:prox_ti_randomize} (\textbf{Random}) with $\lambda=0.001$ (left), $\lambda=0.1$ (center), and $\lambda=10.0$ (right).}
        \label{fig:prox_sort_vs_random}
    \end{figure}
    As shown in~\cref{fig:prox_sort_vs_random}, \textbf{Random} outperformed \textbf{Sort} in most cases.
    \textbf{Sort} sometimes ran faster than \textbf{Random} only when $d$ was very small ($d \le 2^5 =32$).
    Thus, we basically recommend \textbf{Random} (\cref{alg:prox_ti_randomize}) rather than \textbf{Sort} (\cref{alg:prox_ti_sort}) for the evaluation of the proximal operator~\eqref{eq:prox_ti}.

==> Factorization machines with Regularization for Sparse Feature Interactions/impl_details_revised.tex <==
\section{Implementation Details}
    \label{sec:impl}
    In this section, we briefly review and show the implementation details of the existing and proposed algorithms.
    
    \paragraph{$O(d \log d)$ Time Algorithm for Proximal Operator~\eqref{eq:prox_ti}~\citep{filipe2011online}.} \Cref{alg:prox_ti_sort} shows the procedure for solving~\eqref{eq:prox_ti} in $O(d \log d)$ time, where $p_{(i)}$ is the $i$-th largest value of $p_{(\theta)}$ in absolute value; i.e., $|p_{(1)}| \ge |p_{(2)}| \ge \cdots \ge |p_{(d)}|$ and $\forall j \in [d]$ $\exists$ $i \in [d]$ s.t. $p_j = p_{(i)}$.
    \begin{algorithm}[t]
        \caption{Computation of the proximal operator~\eqref{eq:prox_ti} with sorting $\bm{p}$ ($O(d \log d)$).}
        \label{alg:prox_ti_sort}
        \begin{algorithmic}[1]
            \Input{$\bm{p} \in \real^d$, $\lambda \ge 0$}
            \State{$\tilde{\bm{p}} \leftarrow (p_{(1)}, \ldots, p_{(d)})^\top$;}\Comment{$O(d \log d)$}
            \State{$S_0\leftarrow 0$;}
            \For{$j = 1, \ldots, d$}
                \State{$S_j \leftarrow S_{j-1} + \abs{\tilde{p}_j}$;}
            \EndFor
            \State{$S_j \leftarrow S_{j} / (1 + 2\lambda j)$ for all $j \in [d]$;}
            \State{$\theta \leftarrow \max\{j \in [d]: \abs{\tilde{p}_j} - 2 \lambda S_j \ge 0\}$;}
            \State{$q^*_j \leftarrow \sign(p_j) \max \{\abs{p_j} - 2 \lambda S_{\theta}, 0\}$ for all $j \in [d]$;}
            \Output{$\bm{q}^* (= \prox_{\lambda \norm{\cdot}_1^2}(\bm{p}))$}
        \end{algorithmic}
    \end{algorithm}
    
    \paragraph{$O(d)$ Time Algorithm for Proximal Operator~\eqref{eq:prox_ti}~\citep{filipe2011online}.} In fact, the proximal operator~\eqref{eq:prox_ti} can be computed in $O(d)$ time.
    Given $p_{(\theta)}$ (not the index $\theta$, but the value $p_{(\theta)}$), one can compute $S_{\theta}$ in $O(d)$ time: $S_{G_{(\theta)}} \coloneqq \sum_{j \in G_{(\theta)}}|p_j| / (1+2\lambda |G_{(\theta)}|) = S_{\theta}$, where $G_{(\theta)} \coloneqq \{j \in [d]: |p_j| \ge |p_{(\theta)}|\}$ (clearly, $\theta = |G_{(\theta)}|$).
    Thus, even if $\bm{p}$ is not sorted by absolute value, one can compute $\bm{q}^*$ in $O(d)$ time if only $p_{(\theta)}$ is found. Fortunately, one can find $p_{(\theta)}$ in $O(d)$ time in expectation by using the randomized-median-finding-like algorithm~\citep{duchi2008efficient}.
    \Cref{alg:prox_ti_randomize} shows the procedure for computing the proximal operator~\eqref{eq:prox_ti} in $O(d)$ time.
    It finds $p_{(\theta)}$ and computes $S_{\theta}$ by repeating (i) randomly sampling $p_i$ from $\{p_i: j \in C\}$, (ii) determining whether $|p_i| \ge |p_{(\theta)}|$ (although $p_{(\theta)}$ is unknown), and (iii) reducing $C$ in accordance with whether $|p_i| \ge |p_{(\theta)}|$, where $C \subseteq [d]$ is the set of candidates of $\theta$ initialized as $[d]$.
    When $i \in C$ is sampled, the algorithm partitions the candidate index set $C$ into $G \coloneqq \{j \in C: |p_j| \ge |p_i|\}$ and $L\coloneqq \{j \in C: |p_j| < |p_i|\}$ and discards one of them as follows.
    If $|p_i| \ge \lambda S_{G_i}$, where $G_i \coloneqq \{j \in [d]: |p_j| \ge |p_i|\}$, $|p_{(\theta)}|$ is smaller than $|p_i|$, so the algorithm next searches for $p_{(\theta)}$ from $L$ (i.e., it discards $G$).
    In this case, the algorithm updates $S$ and $\theta$ as $S + \sum_{j \in G}|p_j|$ and $\theta +|G|$, respectively (both $S$ and $\theta$ are initially $0$ and are simply desired values when $C=\emptyset$). Maintaining $S$ and $\theta$ reduces the computation cost of $S_{G_i}$: $S_{G_i} = (S + \sum_{j \in G}|p_j|)/[1+2\lambda(\theta + |G|)]$.
    Otherwise (that is, if $|p_i| < 2\lambda S_{G_i}$), the algorithm discards $L$ and sets $C=G_i \setminus \{j \in G: |p_j| = |p_i|\}$ since $|p_{(\theta)}|$ is larger than $|p_i|$.

    \begin{algorithm}[t]
        \caption{Computation of the proximal operator~\eqref{eq:prox_ti} without sorting ($O(d)$)}
        \label{alg:prox_ti_randomize}
        \begin{algorithmic}[1]
            \Input{$\bm{p} \in \real^d$, $\lambda \ge 0$}
            \State{$C \leftarrow [d]$;}\Comment{Candidate index set}
            \State{$S \leftarrow 0$;}
            \State{$\theta \leftarrow 0$;}
            \While{$C \neq \emptyset$}\Comment{Find $p_{(\theta)}$}
                \State{Pick $i \in C$ at random;}
                \State{$G \leftarrow \{j \in C: |p_j| \ge |p_i|\}$}
                \State{$L \leftarrow \{j \in C: |p_j| < |p_i|\}$}
                \State{$S_{G_i} \leftarrow (S + \sum_{j \in G}|p_j|)/(1+2\lambda(\theta + |G|))$}
                \If{$|p_i| - 2\lambda S_{G_i}\ge 0$}\Comment{$|p_i| \ge |p_{(\theta)}|$}
                    \State{$C \leftarrow L$, $S \leftarrow S + \sum_{j \in G}|p_j|, \theta \leftarrow \theta + |G|;$}
                    \Else\Comment{$|p_i| < |p_{(\theta)}|$}
                    \State{$C \leftarrow G\setminus \{j \in G: |p_j| = |p_i|\}$;}
                \EndIf
            \EndWhile
            \State{$S_{\theta} \leftarrow S / (1+2\lambda\theta)$;}
            \State{$q^*_j \leftarrow \sign(p_j) \max \{|p_j| - 2\lambda S_{\theta}, 0\}$ for all $j \in [d]$;}
            \Output{$\bm{q}^* (= \prox_{\lambda \norm{\cdot}_1^2}(\bm{p}))$}
        \end{algorithmic}
    \end{algorithm}
    
    \paragraph{CD Algorithm for Canonical FMs.}~\cref{alg:cd_fm} shows the CD algorithm for objective function~\eqref{eq:objective_fm}.
    The CD algorithm requires the predictions of all training instances $f_n = f_{\mathrm{FM}}(\bm{x}_n; \bm{w}, \bm{P})$ for all $n \in \supp(\bm{x}_{:, j})$ for updating $p_{j, s}$.
    The na\"ive computation of such $f_n$ at each iteration is too costly, so a method for \emph{updating} (\emph{synchronizing}) predictions is essential for an efficient implementation.
    Typically, an efficient algorithm computes and caches $f_n$ for all $n \in [N]$ before starting the optimization and synchronizes them every time a parameter is updated.
    Fortunately, FMs are multi-linear w.r.t $w_1, \ldots, w_d$ and $p_{1,1}, \ldots, p_{d, k}$, so each prediction can be easily synchronized in $O(1)$.
    For $w_j$, the predictions are written as $f_n = x_{n, j}w_j + \mathrm{const}$ for all $n \in [N]$, so $f_n$ are synchronized as $f_n \leftarrow f_n - x_{n, j} \eta \delta$ after updating $w_j$ as $w_j \leftarrow w_j - \eta \delta$.
    To be more precise, the algorithm synchronizes $f_n$ for only $n \in \supp(\bm{x}_{:, j})$ since $f_n$ does not change for all $n \not \in \supp(\bm{x}_{:, j})$.
    For $p_{j, s}$, the predictions are written as $f_n = f'_{n,s}p_{j, s} + \mathrm{const}$, where $f'_{n,s} = x_{n, j}(a_{n,s} - x_{n,j}p_{j,s})$ and $a_{n,s} := \inner{\bm{x}_{n}}{\bm{p}_s}$.
    Thus the algorithm can synchronize $f_n$ as in the case for $w_j$ by caching $a_{n, s}$ for all $n \in [N]$, $s \in [k]$.
    Clearly, the gradient of the loss w.r.t $p_{j, s}$ can be efficiently computed by using $f'_{n,s}$: $\partial \ell (f_n, y_n) / \partial p_{j,s} = \partial \ell(f_n, y_n)/\partial f_n \cdot f'_{n,s}$.
    At each iteration, the algorithm requires $a_{n, s}$ for all $n \in [N]$ and therefore the additional space complexity for caches is $O(N)$ (the algorithm does not require $a_{n,s}$ for all $s \in [k]$ at the same time).
    
    \begin{algorithm}[t]
        \caption{CD algorithm for canonical FMs}
        \label{alg:cd_fm}
        \begin{algorithmic}[1]
            \Input{$\{(\bm{x}_n, \bm{y}_n) \}_{n=1}^{N}$, $k \in \natu_{>0}$, $\lambda_{w}, \lambda_{p} \ge 0$}
            \State{Initialize $\bm{P} \in \real^{d\times k}$, $\bm{w} \in \real^d$;}
            \State{Compute predictions: $f_{n} \leftarrow f_{\mathrm{FM}}(\bm{x}_n;\bm{w}, \bm{P})$ for all $n \in [N]$;}
            \While{not convergence}
                \For{$j=1, \ldots, d$}\Comment{Update $\bm{w}$}
                    \State{$\delta \leftarrow \sum_{i \in \supp(\bm{x}_{:, j})}\ell'(f_n, y_n) x_{n, j}/N + 2\lambda_{w} w_j$};
                    \State{$\eta \leftarrow (\mu \norm{\bm{x}_{:, j}}_2^2/N + 2\lambda_{w})^{-1}$;}
                    \State{$w_j \leftarrow w_j - \eta \delta$;}
                    \State{$f_n \leftarrow f_n -  x_{n,j}\eta \delta$ for all $n \in \supp(\bm{x}_{:, j})$;}
                \EndFor
                \For{$s=1, \ldots, k$}\Comment{Update $\bm{P}$}
                    \State{$a_{n, s} \leftarrow \inner{\bm{x}_n}{\bm{p}_{:, s}}$ for all $n \in [N]$;}\Comment{Cache for updating $\bm{p}_{:, s}$}
                    \For{$j=1, \ldots, d$}
                        \State{$f_{n,s}' \leftarrow x_{n, j} (a_{n,s} - x_{n, j}p_{j, s})$ for all $n \in \supp(\bm{x}_{:, j})$;}
                        \State{$\delta \leftarrow \sum_{i \in \supp(\bm{x}_{:, j})}\ell'(f_n, y_n)\cdot f_{n, s}'/N + 2\lambda_{p} p_{j, s}$;}
                        \State{$\eta \leftarrow [\mu \sum_{n \in \supp(\bm{x}_{:, j})} (f'_{n,s})^2/N + 2\lambda_{p}]^{-1}$;}
                        \State{$p_{j, s} \leftarrow p_{j, s} - \eta \delta$;}
                        \State{$f_{n} \leftarrow f_n - f'_{n, s}\eta \delta$ for all $n \in \supp(\bm{x}_{:, j})$;}
                        \State{$a_{n, s} \leftarrow a_{n, s} - x_{n, j}\eta \delta$ for all $n \in \supp(\bm{x}_{:, j})$;}
                    \EndFor
                \EndFor
            \EndWhile
            \Output{Learned $\bm{P}$ and $\bm{w}$}
        \end{algorithmic}
    \end{algorithm}
    
    \paragraph{SGD for Canonical FMs.}
    \Cref{alg:sgd_fm} shows the SGD algorithm for objective function~\eqref{eq:objective_fm}.
    Since it is almost straightforward, we only describe the \emph{lazy update} technique~\citep{duchi2011adaptive}, which improves the efficiency of the algorithm by leveraging the sparsity of a sampled instance.
    For all $j \not \in \supp(\bm{x}^t)$, where $\bm{x}^t$ is the sampled instance at $t$-th iteration, the gradients of loss function w.r.t $w_j$ and $\bm{p}_j$ are $2\lambda_w w_j$ and $2 \lambda_p \bm{p}_j$, and update rules are $w_j \leftarrow (1-2\eta^t_{w})w_j$ and $\bm{p}_j \leftarrow (1-2\eta^t_{p}) \bm{p}_j$, respectively.
    The lazy update technique enables us to omit updating such parameters and makes the computational cost of each iteration $O(\mathrm{nnz}(\bm{x}_{n})+\mathrm{nnz}(\bm{x}_{n})k)$ while a na\"ive implementation takes $O(d+dk)$.
    Although we hereinafter consider for only $\bm{w}$ for simplicity, the same holds for $\bm{P}$.
    Assume that the algorithm is at $t$-th iteration and $x^t_{j} \neq 0$, and also assume that there exists $t_j < t$ such that $x^{t_j}_j \neq 0$ and $x^{t'}_j = 0$ for all $t_j < t' < t$ (namely, $j$-th feature is $0$ from $(t_j+1)$-th until $(t-1)$-th iteration.
    Then, the value of $w_j$ at $(t-1)$-th iteration, $w^{t-1}_j$, is written as
    \begin{align}
        w^{t-1}_j &= (1-2\eta^{t-1}_w\lambda_w)w^{t-2}_j = \left\{\prod_{t'=t_j+1}^{t-1} (1-2\eta_w^{t'} \lambda_w)\right\} w_j^{t_j} \\
        & =\left\{\frac{\prod_{t'=1}^{t-1} (1-2\eta_w^{t'} \lambda_w)}{\prod_{t'=1}^{t_j} (1-2\eta_w^{t'} \lambda_w)}\right\} w_j^{t_j} =: \frac{\alpha^{t-1}_{w}}{\alpha^{t_j}_{w}} w_j^{t_j}.
    \end{align}
    Therefore, given $\alpha^{t-1}_w$ and $\alpha^{t_j}_{w}$, the algorithm can update $w^t_j$ from $w^{t_j}_j$ in $O(1)$.
    Since $x^{t'}_j = 0$ for all $t' \in \{t_j+1, \ldots, t-1\}$, omitting to update $w_j$ from $(t_j+1)$-th until $(t-1)$-th iteration does not affect the result.
    $\alpha_{w,j}$ in~\cref{alg:sgd_fm} corresponds to $\alpha_w^{t_j}$.
    In our implementation, if $\alpha_w < 10^{-9}$, algorithm updates all $w_j$ and resets $\alpha_w$ and $\alpha_{w,j}$ for all $j \in [d]$ in order to avoid numerical errors.
    The additional space complexity for caches is $O(d)$ (scaling values $\alpha_{w, j}, \alpha_{p,j}$ for all $j \in [d]$).

    \begin{algorithm}[t]
        \caption{SGD algorithm for canonical FMs}
        \label{alg:sgd_fm}
        \begin{algorithmic}[1]
            \Input{$\{(\bm{x}_n, \bm{y}_n) \}_{n=1}^{N}$, $k \in \natu_{>0}$, $\lambda_{w}, \lambda_{p} \ge 0$}
            \State{Initialize $\bm{P} \in \real^{d\times k}$, $\bm{w} \in \real^d$;}
            \State{$t \leftarrow 1;$}
            \State{$\alpha_w, \alpha_p, \alpha_{w,j}, \alpha_{p, j} \leftarrow 1$ for all $j \in [d]$;}\Comment{For lazy update}
            \While{not convergence}
                \State{Sample $(\bm{x}^t, y^t) \in \{(\bm{x}_1,y_1), \ldots, (\bm{x}_N, y_N)\}$;}
                \State{$w_j \leftarrow \alpha_w / \alpha_{w, j} w_j, \ \bm{p}_j \leftarrow \alpha_p / \alpha_{p, j} \bm{p}_j$ for all $j \in \supp(\bm{x}^t)$;}\Comment{Lazy update for regularization term}
                \State{Compute the prediction: $f^t \leftarrow f_{\mathrm{FM}}(\bm{x}^t;\bm{w}, \bm{P})$;}
                \State{$f'_{j, s} \leftarrow x^t_{j}[\inner{\bm{x}^t}{\bm{p}_{:, s}} - x^t_{j}p_{j,s}]$ for all $j \in \supp(\bm{x}^t)$, $s \in [k]$;}
                \State{$L'_{w,j}\leftarrow \ell'(f^t, y^t) \cdot x^t_j + 2\lambda_w w_j$ for all $j \in \supp(\bm{x}^t)$;}
                \State{$L'_{p, j, s} \leftarrow \ell'(f^t, y^t) \cdot f'_{j, s} + 2\lambda_p p_{j, s}$ for all $j \in \supp(\bm{x}^t)$, $s \in [k]$;}
                \State{Compute step size parameter $\eta^{t}_w, \eta^{t}_p$;}
                \State{$w_j \leftarrow w_j - \eta^t_w L'_{w, j}$ for all $j \in \supp(\bm{x}^t)$;}
                \State{$p_{j, s} \leftarrow p_{j, s} - \eta^t_p L'_{p, j, s}$; for all $j \in \supp(\bm{x}^t)$, $s \in [k]$;}
                \State{$\alpha_w \leftarrow (1-2\eta\lambda_w)\alpha_w, \ \alpha_p \leftarrow (1-2\eta\lambda_p)\alpha_p$;}
                \State{$\alpha_{w, j} \leftarrow \alpha_w,\ \alpha_{p, j} \leftarrow \alpha_p$ for all $j \in \supp(\bm{x}^t)$;}
                \State{$t \leftarrow t+1$;}
            \EndWhile
             \State{$w_j \leftarrow \alpha_w / \alpha_{w, j} w_j,\ \bm{p}_j \leftarrow \alpha_p / \alpha_{p, j} \bm{p}_j$ for all $j \in [d]$;}\Comment{Finalize}
            \Output{Learned $\bm{P}$ and $\bm{w}$}
        \end{algorithmic}
    \end{algorithm}

    \paragraph{PBCD Algorithm for Sparse FMs.}
    \Cref{alg:bcd_sfm} shows the PBCD algorithm for sparse FMs with/without the line search~\citep{tseng2009coordinate}, where $\Omega: \real^{d \times k}$ is a sparsity-inducing regularizer.
    The operator $\prox_{\Omega}(\cdot, j)$ in line 18 is the proximal operator for only $j$-th row vector.
    The PBCD algorithm for such sparse FMs updates not $p_{j, s}$ but $\bm{p}_j$ at each iteration and it takes $O(\mathrm{nnz}(\bm{x}_{:, j})k)$ computational cost (if the proximal operator can be evaluated in $O(k)$).
    In this algorithm, we show the two variants for choosing step size $\eta$: using the line search method proposed by~\citet{tseng2009coordinate} and using the Lipschitz constant of the gradient.
    $\sigma, \rho \in (0, 1)$ are hyperparameters for the line search.
    In our experiments, we used the BCD algorithm without the line search.
    The additional space complexity for caches is $O(Nk)$ (caching $\bm{a}_n \in \real^k$ for all $n \in [N]$ requires $O(Nk)$ and caching $\bm{q}, \bm{\delta}, \bm{d} \in \real^{k}$ requires $O(k)$).
    Some sparse regularizers (e.g, CS regularizer) require some additional caches and how to compute/use caches depends on the regularizer.
    Moreover, in the case of using the line search, some regularizers might also require a non-obvious efficient incremental evaluation method (i.e., na\"ive computation of $\Omega(\cdot)$ might take a high computational cost that is prohibitive at each line search iteration).
    
    \begin{algorithm}[t!]
        \caption{PBCD algorithm for sparse FMs}
        \label{alg:bcd_sfm}
        \begin{algorithmic}[1]
            \Input{$\{(\bm{x}_n, \bm{y}_n) \}_{n=1}^{N}$, $k \in \natu_{>0}$, $\lambda_{w}, \lambda_{p}, \tilde{\lambda}_{p} \ge 0$, optional: $\sigma, \rho \in (0, 1)$ (for line search)}
            \State{Initialize $\bm{P} \in \real^{d\times k}$, $\bm{w} \in \real^d$;}
            \State{Compute predictions: $f_{n} \leftarrow f_{\mathrm{FM}}(\bm{x}_n;\bm{w}, \bm{P})$ for all $n \in [N]$;}
            \While{not convergence}
                \State{Optimize $\bm{w}$ and update caches as in canonical FMs;}
                \State{$\bm{a}_{n} \leftarrow \bm{P}^\top \bm{x}_{n} \in \real^{s}$ for all $n \in [N]$;}\Comment{Cache for update $\bm{P}$}
                \If{Perform line search}
                    \State{$L \leftarrow \sum_{n=1}^N \ell(f_n, y_n)/N + \lambda_{p} \norm{\bm{P}}_2^2 + \tilde{\lambda}_{p} \Omega(\bm{P})$;}\Comment{Objective value used in line search}
                \EndIf
                \For{$j=1, \ldots, d$}
                    \State{$\bm{f}'_n \leftarrow x_{n, j}(\bm{a}_n - x_{n, j}\bm{p}_{j})$ for all $n \in \supp(\bm{x}_{:, j})$;}
                    \State{$\nabla_{\bm{p}_{j}}\ell_n \leftarrow \ell'(f_n, y_n) \bm{f}'_n$ for all $n \in \supp(\bm{x}_{:, j})$};
                    \State{$\bm{d} \leftarrow (\sum_{n \in \supp(\bm{x}_{:, j})}\nabla_{\bm{p}_{j}}\ell_n)/N + 2\lambda_{p} \bm{p}_{j}$;}
                    \If{Perform line search}
                        \State{$\eta^{-1} \leftarrow \max_{s \in [k]} \{2\lambda_{p} + \sum_{n \in \supp(\bm{x}_{:, j})}\ell''(f_n, y_n)(\partial f_{\mathrm{FM}}(\bm{x}_n)/\partial p_{j,s})^2/N\}$;}
                    \Else
                        \State{$\eta^{-1} \leftarrow 2\lambda_p + \mu \sum_{n \in \supp (\bm{x}_{:, j})} \norm{\nabla_{\bm{p}_j} \ell_n}_2^2 / N$;}
                    \EndIf
                    \State{$\bm{q} \leftarrow \prox_{\tilde{\lambda}_{p}\eta \Omega}(\bm{P} - \eta \bm{e}^d_j \bm{d}^\top; j)$;\Comment{Apply for only $j$-th row vector}}
                    \State{$\bm{\delta} \leftarrow \bm{p}_{j} - \bm{q}$;}
                    \If{Perform line search}
                        \State{$L_{\mathrm{new}}\leftarrow L + \sum_{n \in \supp(\bm{x}_{:, j})}[\ell(f_n-\inner{\bm{f}'_n}{\bm{\delta}}, y_n)-\ell(f_n, y_n)]/N$;}
                        \State{$L_{\mathrm{new}}\leftarrow L_{\mathrm{new}} + \lambda_{p} (\norm{\bm{q}}_2^2 - \norm{\bm{p}_j}_2^2) + \tilde{\lambda}_{p}\left[\Omega(\bm{P} - \bm{e}^d_{j} \bm{\delta}^\top) - \Omega(\bm{P})\right]$;}
                        \State{$\alpha \leftarrow 1$;}
                        \While{not $L_{\mathrm{new}} - L \le \sigma \alpha \{-\inner{\bm{d}}{\bm{\delta}} + \tilde{\lambda}_p[\Omega({\bm{P} -\bm{e}^d_j \bm{\delta}^\top})-\Omega(\bm{P})]\}$}
                            \State{$L_{\mathrm{new}}\leftarrow L_{\mathrm{new}} + \sum_{n \in \supp(\bm{x}_{:, j})}\left[\ell(f_n-\inner{\bm{f}'_n}{\alpha\rho\bm{\delta}}, y_n) - \ell(f_n-\inner{\bm{f}'_n}{\alpha\bm{\delta}}, y_n)\right]/N$;}                    \State{$L_{\mathrm{new}}\leftarrow L_{\mathrm{new}} + \lambda_{p} \left[\norm{\bm{p}_j-\alpha\rho\bm{\delta}}_2^2 - \norm{\bm{p}_j-\alpha\bm{\delta}}_2^2\right]$;}
                            \State{$L_{\mathrm{new}}\leftarrow L_{\mathrm{new}} + \tilde{\lambda}_{p}\left[\Omega(\bm{P} - \alpha \rho \bm{e}^d_{j} \bm{\delta}^\top) - \Omega(\bm{P} - \alpha \bm{e}^d_{j} \bm{\delta}^\top)\right]$;}
                            \State{$\alpha \leftarrow \alpha \rho$;}
                        \EndWhile
                    \State{$L \leftarrow L_{\mathrm{new}}$;}
                    \State{$\bm{\delta} \leftarrow \alpha \bm{\delta}$;}
                    \EndIf
                    \State{$\bm{p}_{j} \leftarrow \bm{p}_j - \bm{\delta}$;}
                    \State{$\bm{a}_{n} \leftarrow \bm{a}_n - x_{n,j}\bm{\delta}$ for all $n \in \supp(\bm{x}_{:, j})$;}
                    \State{$f_{n} \leftarrow f_n -  \inner{\bm{f}'_n}{\bm{\delta}}$ for all $n \in \supp(\bm{x}_{:, j})$;}
                \EndFor
            \EndWhile
            \Output{Learned $\bm{P}$ and $\bm{w}$}
        \end{algorithmic}
    \end{algorithm}
    
    \paragraph{PSGD Algorithm for Sparse FMs.}
    The extension of~\cref{alg:sgd_fm} to PSGD algorithm for sparse FMs is straightforward: evaluates a proximal operator for a sparse regularization after updating $\bm{P}$ at each iteration.
    For $\tilde{\ell}_{1,2}^2$-sparse FMs (TI-sparse FMs), all parameters must be the latest values at each iteration, i.e., a lazy update technique cannot be used.

    \paragraph{Extension to HOFMs.}
    Here we describe the extension of above described algorithms for $M$-order HOFMs.
    The extended algorithms update $\bm{w}$, $\bm{P}^{(2)}, \ldots, \bm{P}^{(M)}$ sequentially.
    HOFMs are also multi-linear w.r.t $\bm{w}, \bm{p}_{1}^{(2)}, \ldots, \bm{p}_{d}^{(M)}$ (and clearly $w_{0}, \ldots, w_{d}, p_{1,1}^{(2)}, \ldots, p_{d, k}^{(M)}$)~\citep{blondel2016higher} and thus the output of HOFMs are written as $f_{\mathrm{HOFM}}^M(\bm{x}) = \inner{\bm{\theta}}{\nabla_{\bm{\theta}}f_{\mathrm{HOFM}}^M(\bm{x})} + \mathrm{const}$ for a parameter $\bm{\theta} \in \{\bm{w}, \bm{p}_1^{(2)}, \ldots, \bm{p}_d^{(M)}\}$.
    Given $\nabla_{\bm{\theta}} f_{\mathrm{HOFM}}^M(\bm{x})$, the parameter $\bm{\theta}$ and predictions can be updated efficiently in both CD (updates only one element in $\bm{\theta}$) and BCD algorithms.
    For each case, $\partial f_{\mathrm{HOFM}}^M(\bm{x})/\partial \theta_j$ is written as
    \begin{align}
        \frac{\partial f_{\mathrm{HOFM}}^M(\bm{x})}{\partial \theta_j} = \begin{cases}
        x_j & \text{if } \theta_j = w_j, \ j \in [d],\\
        x_j\anova^{m-1}(\bm{x}_{\lnot j}, (\bm{p}_{:, s})_{\lnot j}) & \text{if } \theta_j = p_{j, s}^{(m)},\ m \in \{2, \ldots, M\},\ j \in [k],
        \end{cases}
    \end{align}
    where $\bm{x}_{\lnot j} \in \real^{d-1}$ is the $(d-1)$-dimensional vector with $x_j$ removed.
    Thus, the replacement of  $f'_{n, s}$ in~\cref{alg:cd_fm} ($\bm{f}'_{n}$ in~\cref{alg:bcd_sfm}) with $\partial f_{\mathrm{HOFM}}^m(\bm{x}_n)/\partial p_{j,s}^{(m)}$ ($\nabla_{\bm{p}_j^{(m)}} f_{\mathrm{HOFM}}^m(\bm{x}_n)$) produces the CD (BCD) algorithm for HOFMs.
    \Cref{alg:sgd_fm} can be also extended to the SGD algorithm for HOFMs similarly.
    Here, the issue is clearly how to compute $\partial f_{\mathrm{HOFM}}^M(\bm{x}_n)/\partial p_{j,s}^{(m)}$ efficiently.
    Fortunately,~\citet{blondel2016higher} and~\citet{atarashi2020link} proposed efficient computation algorithms for $\anova^{m-1}(\bm{x}_{\lnot j}, (\bm{p}_{:, s})_{\lnot j})$.
    For more detail, please see~\citep{blondel2016higher,atarashi2020link}.

